Hera: A Heterogeneity-Aware Multi-Tenant Inference Server for Personalized Recommendations

While providing low latency is a fundamental requirement in deploying recommendation services, achieving high resource utility is also crucial in cost-effectively maintaining the datacenter. Co-locating multiple workers of a model is an effective way to maximize query-level parallelism and server throughput, but the interference caused by concurrent workers at shared resources can prevent server queries from meeting its SLA. Hera utilizes the heterogeneous memory requirement of multi-tenant recommendation models to intelligently determine a productive set of co-located models and its resource allocation, providing fast response time while achieving high throughput. We show that Hera achieves an average 37.3% improvement in effective machine utilization, enabling 26% reduction in required servers, significantly improving upon the baseline recommedation inference server.

==> tex/discussion.tex <==
\section{Related Work}
\label{sect:discussion}

Because of the rapidly increasing complexity of DNN-based ML algorithms, the
computer architecture community has witnessed a surge of interest in ML
accelerator architectures with a strong emphasis on accelerating CNNs, RNNs,
            and
            MLPs~\cite{diannao,dadiannao,shidiannao,pudiannao,du:2015:micro,minerva,dnn_pim_reram,eyeriss,cambricon,isacc,neurocube,redeye,tabla,dnnweaver,intel:2017:fpl,gao:2017:tetris,intel:2018:fpga,rhu:2016:vdnn,song:2015:eie,cnvlutin,cambriconx,stripes,bitpragmatic,intel:2017:icassp,intel:2017:fpga,whatmough:2017:isscc,whatmough:2017:hotchips,scnn,bittactical,rhu:2018:cdma,tpu1}.
            As the focus of these prior work is on designing a single NPU in
            isolation, little attention has been paid in \emph{how} the ML
            inference server collects the batched inputs to feed it into these
            NPU architectures. The key objective of our \lazyb design is to
            study the implication of batching on the system-level latency,
            throughput, and QoS which is a rare contribution in our community
            given its primary focus on ML accelerator design so far.  In
            general, the contributions and intuitions behind our proposed
            \lazyb architecture can readily be applied to prior NPU proposals
            and is hence orthogonal to the closely related prior work above.


